Orchestrating the Development Lifecycle of Machine Learning-Based IoT Applications: A Taxonomy and Survey

Machine Learning (ML) and Internet of Things (IoT) are complementary advances: ML techniques unlock complete potentials of IoT with intelligence, and IoT applications increasingly feed data collected by sensors into ML models, thereby employing results to improve their business processes and services. Hence, orchestrating ML pipelines that encompasses model training and implication involved in holistic development lifecycle of an IoT application often leads to complex system integration. This paper provides a comprehensive and systematic survey on the development lifecycle of ML-based IoT application. We outline core roadmap and taxonomy, and subsequently assess and compare existing standard techniques used in individual stage.

==> figuresTex/fig-datatype.tex <==
\begin{figure}[hbt]
\centering
\includegraphics[width=4.0in, height=3in]{figuresTex/figures/data_type.pdf}
 \caption{Data generation in IoT system}
\label{fig:datatype}
\end{figure}

==> figuresTex/fig-model-fault.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=5.0in, height=2.5in]{figuresTex/figures/neural.pdf}
 \caption{A $2$ layer neural network, where $Y_{i}^{(j)}$ represent a computation node (neuron), and the synaptic weight of synapse $w_{i}^{(j)}$ which transmits the messages between two neurons. The dotted nodes represent the inputs and outputs which are not considered in the network.}
\label{fig:fault}
\end{figure}

==> figuresTex/fig-taxonomy.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=5.0in, height=7in]{figuresTex/figures/taxonomy_1.pdf}
 \caption{A taxonomy in orchestrating ML-based IoT application development lifecycle}
\label{fig:taxonomy}
\end{figure}



==> overview.tex <==
\section{Overview and Background}
\label{sec:overview}

%Large-scale big data analytics tends to rely on more computing resources and
%higher parallelization at a centralized location to perform the exact and
%low-latency data analysis.
%% In contrast, approxmiate computing enables a systematic trade-off between the
%% analysis accuracy and scalability.
%Apparently, processing the entire data set can provide analysts with confidence
%on their analysis results. However, it is neither necessary nor feasible to
%obtain the exact statistics all the time. For instance, the analysts sometimes
%need to run different ad hoc queries to obtain quick update on viral trends or
%events. In such a case, 100\% accurate analysis may not be too critical, and it
%may be entirely acceptable to trade the accuracy for desirable latency
%performance.  \projecttitle aims to provide such flexibility that the existing
%systems lack; it employs sampling and controls the population of a subset of the
%data in a dynamic fashion to meet the requirements of the analysts.

% This section gives an overview of \projecttitle and a brief background on the
% technical building blocks.

\input{figuresTex/fig-system-overview.tex}

\subsection{System Overview}
\label{subsec:overview}

\projecttitle builds on two design concepts: hierarchical processing and
approximate computing. In \projecttitle, a wide variety of devices or sensors
(so-called IoT devices) generate and send data streams to regional edge
computing nodes geographically close to themselves. The edge computing
clusters managed by local ISPs or content providers sample only a subset of the
input data streams and forward them to larger computing facilities such as datacenters. The data streams, again sampled at the datacenters, can be further
forwarded to a central location, where a user-specified query is executed and
the query results are produced for global-level analysis. These computing
clusters spread across the globe form a logical stream processing pipeline as a
tree, which is collectively called \projecttitle. \figref{fig:overview} presents
the high-level structure of the system.

% In \projecttitle, the input data stream combines multiple \emph{sub-streams},
% each of which is a collection of data items from an individual data source.
% In other words, the input data stream consists of data items from diverse data
% sources.

% Our \projecttitle system consists of multiple nodes that form a logical
% aggregation tree, where each node is a computing entity (ranging from a single
% server to even a data center). First, the leaf nodes (e.g., regional edge
% computing infrastructures) in the aggregation tree receive the sub-streams
% from diverse data sources. Afterwards, the leaf nodes process such sub-streams
% and forward them to the upper-layer nodes (e.g., continental computing
% infrastructures). Each node in the aggregation tree follows such a process, so
% that finally the root node (the central computing infrastructure) in the tree
% can execute a user-specified query and produce the query results.
% \projecttitle applies a sliding-window computational model~\cite{slider},
% whereby the window slides over the input data stream and different windows do
% not overlap.

The design choice of \projecttitle, i.e., combining approximate computing and
hierarchical processing, naturally enables the processing of the input data
stream within a specified resource budget. 
% \projecttitle makes use of approximate computing by transferring and
% processing only a subset of data items received at each node, and
On top of this feature, \projecttitle produces an approximate query result with
rigorous error bounds. In particular, \projecttitle designs a parallelizable
online sampling technique to select and process a subset of data items, where
the sample size can be determined based on the resource constraints at each node
(i.e., computing cluster), without any cross-node coordination.




Altogether, \projecttitle achieves three goals.
\begin{itemize}
\item \textbf{Resource efficiency.} \projecttitle utilizes computing and
  bandwidth resources efficiently by sampling data items at each individual node in the logical tree.  If we were to sample data items only at a node where the query
  is executed, all the computing and bandwidth resources used to process and forward the unused data items would have been wasted.

% \item \textbf{Autonomy.} Each node individually determines the level of
%   sampling based on its local resource constraints. This autonomy allows
%   \projecttitle to quickly adapt to the changing conditions regarding the
%   available resources (e.g., computing and bandwidth resources).  Arguably,
%   an ideal centralized orchestration might enable the optimal resource
%   utilization; however, such an approach would need to assume the accurate
%   and real-time knowledge of the available resources across all the nodes.
%   This is impractical especially in an IoT setting where computing nodes
%   operate in a geographically distributed manner.

\item \textbf{Adaptability.} The system can adjust the degree of sampling based
  on resource constraints of the nodes. While the core design is agnostic to the
  ways of choosing the sample size, i.e., whether it is centralized or
  distributed, this adaptability ensures better resource utilization.

\item \textbf{Transparency.} For an analyst, the system enables computation over
  the distributed data in a completely transparent fashion. The analyst does not
  have to manage computational resources; neither does she require any code
  changes to existing data analytics application/query.
\end{itemize}


% \subsection{Design Assumptions} 
% \label{subsec:assumptions}

% The design of \projecttitle is based on the following three assumptions. 

% \begin{itemize}
% \item[1.] We assume there exists a virtual cost function which translates a given query budget (such as the user-specified latency/throughput/accuracy guarantees) into the appropriate sample size.

% \item[2.] We assume the input data stream can be stratified according to the data sources, and the data items from each source (i.e., a sub-stream) follow the same distribution.

% \item[3.] We assume a time-based sliding window.  With different data arrival rates,  the number of data items within a window may vary accordingly. 
% \end{itemize}


\subsection{Technical Building Blocks}
\label{sec:preliminaries}

%\projecttitle is required to support various queries such as sum, average,
%standard deviation, etc. While there are many sketch algorithms~\cite{cormode05}
%and sampling techniques~\cite{estan03, hohn03}, they are ill-suited for our
%target use cases as they tend to lose statistics on low-volume streams. Thus,
%\projecttitle excludes these approaches in its design. Instead, 

\projecttitle relies on two sampling techniques as the building blocks: stratified
sampling~\cite{stratified-sampling} and reservoir sampling~\cite{reservoir}
because the properties of the two allow \projecttitle to meet its needs.

\subsubsection{Stratified Sampling}

A sub-stream is the data items from a source. In reality, sub-streams from
different data sources may follow different distributions. Stratified sampling
was proposed to sample such sub-streams fairly. Here, each sub-stream forms a
stratum; if multiple sub-streams follow the same data distribution, they can be
combined to form a stratum. For clarity and coherence, hereafter, we still use
sub-stream to refer to a stratum.

Stratified sampling receives sub-streams from diverse data sources, and performs the sampling (e.g., simple random sampling~\cite{sampling-3} or other types of sampling) over each sub-stream independently.
In doing so, the data items from each sub-stream can be fairly selected into the sample.  Stratified sampling reduces sampling error and improves the precision of the sample.  It, however, works only in a situation where it can assume the knowledge of the statistics of all sub-streams (e.g., each sub-stream's length).  This assumption on prior knowledge is unrealistic in practice.



\subsubsection{Reservoir Sampling}

Reservoir sampling is often used to address the unrealistic assumption aforementioned in stratified sampling.  It works without the prior knowledge of all the sub-streams.  Suppose a system receives a stream consisting of an unknown number of data items.  Reservoir sampling maintains a reservoir of size $R$, and wants to select a sample of (at most) $R$ items uniformly at random from the unbounded data stream.  Specifically, reservoir sampling keeps the first-received $R$ items in the reservoir.  Afterwards, whenever the $i$-th item arrives ($i>R$), reservoir sampling keeps this item with probability of $N/i$ and then randomly replaces one existing item in the reservoir.  In doing so, each data item in the unbounded stream is selected into the reservoir with equal probability.  Reservoir sampling is resource-efficient; however, it could mutilate the statistical quality of the sampled data items in the reservoir especially when the input data stream combines multiple sub-streams with different distributions.  For example, the data items received from an infrequent sub-stream could easily get overlooked in reservoir sampling.



%\textbf{Importance of considering the sampling rate of each edge node:}
%For a query $Q1$ calculates the mean of collected data from $D1$ to $D6$ can be defined as:
%\begin{equation}
%\footnotesize
%SUM(WE4(a1+a2+a3)+WE5(a4+a5)+WE3*a6)=SUM(SE1)+error
%\end{equation}
%Obviously, the sampling rate of each edge node may affect of the $error$. 
%Firstly, we are not considering the influence of the bandwidth between each node, and make the assumption that the window of the destination node includes all data items from source nodes. For example, the data items in $WE2$ equals to the data items of $SE5+SE4$. 
%Therefore, in $SE1$ the number of the items from $D1$ is $SE1_{D1}=WE4*a1*P_{E4}*P_{E2}*P_{E1}$, where $P_i$ is the sampling rate of edge node $i$. Similarly, the sample of $D6$ is $SE1_{D6}=WE3*a6*P_{E3}*P_{E1}$.  Sum of $SE1$ is:
%\begin{equation}
%SUM(SE1)=\sum_{i=1}^{6} SUM(SE1_{Di})
%\end{equation}
%
%To achieve the unbiased sampling, the proportion of the data items from different sources in $SE1$ must be the same as that are collected from edge devices. For the given example, the proportion of $D1$ from the original data is (assuming $WE4=WE5=WE3$ ): 
%\begin{equation}
%\label{ori_prop}
%prop(D1)= \frac{a1}{\sum_{i=1}^{6} ai}; \; 
%\end{equation}
%and that in $SE1$ is:
%\begin{equation}
%\footnotesize
%\begin{split}
%prop(SE_{D1})= &\frac{a1*P_{E4}*P_{E2}*P_{E1}}{(a1+a2+a3)*P_{E4}*P_{E2}*P_{E1}+(a4+a5)*P_{E5}*P_{E2}*P_{E1}+a6*P_{E3}*P_{E1}} \\
%			=& \frac{a1*P_{E4}*P_{E2}}{(a1+a2+a3)*P_{E4}*P_{E2}+(a4+a5)*P_{E5}*P_{E2}+a6*P_{E3}}
%\end{split}
%\end{equation}
% 
%Therefore, $prop(D1)$ should equal to $prop(SE_{D1})$. 
%
%The following introduces a tree based method to solve the sampling rate problem. 
%Before going the details of the method, we first propose a simple rule for assigning the sampling rates:
%
%\begin{itemize}
%
%	\item From root to leaves, every node from the same level must have the same \emph{path value};  \emph{path value} is the product of the sampling rates from the given node until any of its leaves.   
%\end{itemize}
%
%For the given example, the rule can be translated as: $P_{E4}*P_{E2}*P_{E1}=P_{E5}*P_{E2}*P_{E1}=P_{E3}*P_{E1}=P$, where $P$ is the total sampling rate for a subStream. 
%If we assign $P=25\%$ and $P_{E1}=50\%$, we therefore can have $P_{E3}=50\%$ based on given the rule. Since $P_{E3}$ equals to $50\%$, we then have $P_{E4}*P_{E2}=P_{E5}*P_{E2}=P_{E3}=50\%$, so we can assign $P_{E2}=80\%$, and $P_{E4}$ and $P_{E5}$ will be $62.5\%$.


%\textcolor{blue}{zy: in "streamApprox", the stratified sampling is used to signed the weight to each sub-stream, based the proportion the sub-stream. 
%The reason that streamApprox does not need to consider the sampling rate is that all subStreams are sampled in the same rate randomly, which will not change the proportion of the sub-streams.}

%\textbf{Importance of considering bandwidths between edge nodes:}
%Geo-Distributed system naturally has various bandwidths which may also cause  the proportion of change of the sampled data comparing with original data.
%
%Recalling the same example in Figure~\ref{fig:aggTree}, we however do not consider the affect of sampling rate, assuming the sampling method is turned off in each edge node. 
%In $E1$, the delivered data items from $D1$ is: 
% \begin{equation}
%\footnotesize
%SE1_{D1}^{*}= \argmin (\{\{a1*WE4\}, \{a11*WE2*\frac{a1}{a1+a2+a3}\}, \{a21*WE1*\frac{a11*a1(a11+a12)}{a1+a2+a3}\}\})
%\end{equation}
%
%Again, we assume that the window size of \emph{first} edge nodes (directly connected with edge devices) are the same ($WE4=WE5=WE3$). The proportion of $D1$ from original data is the same as shown equation~\ref{ori_prop}. However, proportion of $D1$ in $SE1$ is:
%   \begin{equation}
%\footnotesize
%prop(SE1_{D1}^{*})= \frac{SE1_{D1}^{*}}{(a21+a13)*WE1}
%\end{equation}
%
%Therefore, the bandwidths between edge nodes will also significantly influence the proportion of the subStream in the sampled data.   
%%The state-of-the-art distributed stream processing systems can be classified in two prominent categories:  {\em (i)} batched stream processing model, and {\em (ii)}  pipelined stream processing model. These systems offer three main advantages: (a) efficient fault tolerance, (b) ``exactly-once'' semantics, and (c) unified programming model for both batch and stream analytics. {\em Our proposed algorithm for approximate computing is generalizable to both stream processing models, and preserves their advantages.}
%%
%%
%%\myparagraph{Batched stream processing model} In this computational model, an input data stream is divided into small batches using a predefined batch interval, and each such batch is processed via a distributed data-parallel job. Apache Spark Streaming~\cite{spark-streaming} adopted this model to process input data streams. While this model is widely used for many applications, it cannot adapt to the cases where low-latency is critical since this model waits for the batching to complete before processing the batch. Sampling the input data stream in a continuous ``on-the-fly'' fashion can be challenging to address in this computational model. However, \projecttitle overcomes this challenge by  performing sampling operations before the batches are formed.
%%
%%
%%\myparagraph{Pipelined stream processing model} In contrast to the batched stream processing model, the pipelined model streams each data item to the next operator as soon as the item is ready to be processed without forming the whole batch. Thus, this model achieves low latency. Apache Flink~\cite{flink} implements the pipelined stream processing model to support a truly native stream processing engine. \projecttitle can adopt this computational model easily by sampling the input data stream in an online manner.
%%
%%
%%Note that both stream processing models support the sliding window computation~\cite{slider}. The processing window slides over the input stream, whereby the newly incoming data items are added to the window and the old data items are removed from the window. The number of data items within a sliding window may vary in accordance to the arrival rate of data items.
%
%%\projecttitle adopts the {\em batched stream processing} model~\cite{spark-streaming}, where an input data stream is divided into small batches of configurable sizes, and each such batch is processed via a distributed data-parallel job.
%%, similar to Apache Spark. 
%%Importantly, note that \projecttitle's sampling operates in a continuous ``on-the-fly" fashion, and the number of data items processed in a batch are a subset of the stream data (chosen based on the sample size).
%
%%More specifically, \projecttitle's design is based on the sliding window computation~\cite{slider}.  The processing window slides over the input stream, whereby the newly incoming data items are added to the window and the old data items are removed from the window.  Note that, in this computational model, the number of data items within a sliding window may vary in accordance to the arrival rate of data items.
%
%
%
%%This batched stream processing model offers three main advantages over the trigger-based processing model~\cite{d-streams}: (a) efficient fault tolerance based on re-computation of failed tasks instead of using a synchronized replication protocol, (b) ``exact-once'' semantics  for processing data items instead of weaker semantics such as ``at least once'' or ``at most once'', and (c) single programming model for both batch and stream analytics. %Given these advantages, the batched streaming model is widely adopted by many stream processing frameworks including Spark Streaming~\cite{spark-streaming},  Flink~\cite{flink}, TimeStream~\cite{timestream}, Trident~\cite{trident}, MapReduce Online~\cite{hop}, Comet~\cite{comet}, and NOVA~\cite{nova}.
%
%
%
%
%
%
%
%%\subsection{Design Assumption} 
%%\label{sec:assumptions}
%%%
%%\projecttitle is based on the that there exists a cost function which translates a given query budget (such as the expected latency/throughput guarantees, or the required accuracy level of query results) into the appropriate sample size. We discuss possible means to design such a cost function  in~\S\ref{sec:discussion}.
%%
%%%
%%
%
%\subsection{Design Assumptions} 
%\label{subsec:assumptions}
%%
%\projecttitle is based on the following assumptions.  We discuss the possible means to reduce these assumptions in~\S\ref{sec:discussion}. %, whereas the third assumption is the default configuration for aforementioned stream processing systems.
%
%\begin{itemize}
%\item[1.] We assume there exists a virtual cost function which translates a given query budget (such as the expected latency/throughput guarantees, or the required accuracy level of query results) into the appropriate sample size.
%
%\item[2.] We assume that the input stream is stratified based on the source of data items, i.e., the data items from each sub-stream follow the same distribution and are mutually independent. Here, a \textit{stratum} refers to one sub-stream. If multiple sub-streams have the same distribution, they are combined to form a stratum. 
%
%\item[3.] We assume a time-based window length.  Based on the arrival rate,  the number of data items within a window may vary accordingly. Note that this assumption is consistent with the sliding window APIs in the aforementioned stream processing systems.
%%We assume that each sub-stream is stratified based on the source of event, i.e., the data items in each sub-stream follow the same distribution, and are independently distributed. Here a \textit{stratum} refers to one sub-stream. If multiple sub-streams have the same distribution, they are combined to form a stratum.
%
%\end{itemize}
%
%%Lastly, we assume a time-based window length, and based on the arrival rate,  the number of data items within a window may vary accordingly. Note that this assumption is consistent with the sliding window APIs in the aforementioned stream processing systems.
%
%\input{preliminaries}


% \textbf{How to sample items in a multi-level StreamApprox approach with
%   bandwidth constraint.}


==> selection.tex <==
\section{Resource selection}
\label{sec:selection}

==> specification.tex <==
\section{Application specification}
\label{sec:specification}
%\zy{I have rewritten everything for this section. However, the contents is not good enough. Maybe Dev can add more. }
%
%The user specification describes the user's requirements and the constraints for developing a system. 
%%They are written by the system owner and end users with input from quality assurance. 
%%Based on the documented requirements, the developer or project manager creates a blueprint to develop the system for their users. 
%Considering a ML-based IoT application, the requirements include the specific performed tasks, the Quality of Service (QoS), the monetary cost, and the constraints of the available computing resources including both hardware and software. 
% 
% To develop a ML-based IoT application, we must consider the specific behaviors or functions that the application can provided. For example, the \emph{smart traffic routing} system mentioned in \S \ref{sec:smartcity} uses cameras to monitor the road traffic. The ``car counting'' function running on each camera is a functional requirement. In ML-based IoT application, these functional are implemented and performed through various ML models. These models are executed in the complex IoT environments. To simply the development and deployment of these models, the ML tasks and the underlying infrastructure must be specified  with optimization for performance and accuracy. The following investigates the specification languages for declarative ML tasks in IoT applications and  declarative computing resources for running these applications.
 
 
%  \subsection{Declarative Machine Learning}\label{sec:declarative-ML}
%  
%  Declarative ML aims to use high-level language to specification of ML tasks which separates the application from the underlying data representation, model training and its computing resources. To be precise, there are \emph{three} general properties of declarative ML.  
% First, the high-level specification only considers the data types of input, intermediate results and output, and they are exposed as abstract data types without considering the physical representation of the data and how the data is processed by the underlying ML models. 
% Second, the ML tasks or models are specified as high-level operations through well-defined semantics. In the specification the basic operation primitives and their expected accuracy levels (or confidence interval) are defined. 
% Based on the operation semantics, the systems for declarative ML can select the feature and underlying ML models manually or automatically and optimize the performance and accuracy of the selected models for varying data characteristics and runtime environments. Notably, the selection is based the underlying models that are already available, provided as the services.    
% Finally, the correctness of the ML models must be satisfied when a given model produce the equivalent results in any computing resources with the same input data and configurations. 
% As a result, the declarative ML provides the possibility of executing the ML models over various hardware and  computation platforms (such as Apache Spark) without any changes.
% 
% SystemML \cite{boehm2016systemml} is an implementation of declarative ML on Apache Spark, which specifies the ML models as abstract data types and operations, independent of their implementation through a domain-specific language. The system is able to specify  a majority of ML models:  matrix factorizations, dimensions reduction, survival models for training and scoring, classification, descriptive statistics, clustering and regression. 
%Moreover, TUPAQ \cite{sparks2015automating} utilizes the declarative ML to describe the supervised learning ML algorithms. The description includes the types of models such as SVM, decision tree, etc. and the models associated hyper-parameters (e.g., the maximum depth of a decision tree). Based on the description, the input data, and some stopping criterion, TUPAQ aims to find and train the ``best'' model which make accurate predictions. 
%Columbus \cite{zhang2016materialization} uses a high-level, declarative constructs to capture models like linear and logistic
%regression, SVM, lasso etc, to achieve the goal of data and computation reuse. 
%
%As a result, the state-of-the-art research show that declarative ML utilize language specification and modeling technologies to describe the ML models for the purposes of automated model and feature selection, performance and resource optimization, model and data reuse etc.  Also, declarative ML can help for the deployment and composition of ML models, which will be detailed in \S \ref{sec:deployment}.
%
%
% \subsection{Declarative Computing Resources}\label{sec:declarative-resource}
% 
 
 

 

%\subsection{Requirement Specification}
%\label{sec:Requirement Specification}
%%Requirement specification, also known as software requirement specification (SRS), is a description of software system to be developed. \zy{need to write one more line}
%Requirement specification or software requirement specification (SRS) is a document that describes the development of a system or an application. It involves a variety of expected functionalities from the customer. Moreover, the customer has the requirements to be aware of the performance of these functionalities. As a result, the requirement specification can be categorized as \emph{functional requirements} and \emph{non-functional requirements}. 
%The requirement specification is a crucial task because the heterogeneous for IoT (from hardware platforms to application protocols) implies a critical need for a multi-layered architecture for IoT application. As a consequence, the requirements may be specified differently regarding each layer of the architecture stack. 
%Compared to the traditional cloud based application, ML-based IoT application involves more types of computing resources, programming languages/frameworks and are deployed in dynamic and uncertain environments. However, the classic method \cite{van2001goal} can still be leveraged to categorize SRS for the ML-based IoT applications. The two categories, \emph{functional requirements} and \emph{non-functional requirements} are discussed below.
%Although the ML-based IoT applications involve more types of computing resources, programming language/frameworks and are deployed in dynamic and uncertain environments, compared to traditional cloud based application, we still follow the classic method \cite{van2001goal} to categorize the requirements of the ML-based IoT applications into two broad categories: \emph{functional requirements} and \emph{non-functional requirements}.

%\subsubsection{Functional Requirements}
%\label{sec:Functional Requirements}
%Functional requirements define specific behaviors or functions of an application. It is very specific to the application itself.  For example, the \emph{smart traffic routing} system mentioned in \S \ref{sec:smartcity} uses cameras to monitor the road traffic. The ``car counting'' function running on each camera is a functional requirement. In ML-based IoT application, these functional requirements are implemented with the ML models and will be detailed in \S \ref{sec:training}.
%
%\subsubsection{Non-Functional Requirements}
%\label{sec:Non-Functional Requirements}
%Non-functional requirements specify the criteria used to evaluate the performance of a system, rather than the specific behaviors~\cite{glinz2007non}. 
%In this paper, we consider the QoS and budget constraint as the NFR of a ML-based IoT application.
%NFR are also knows as Quality of Service (QoS) or Service level requirements or quality attributes or constraints or system capabilities.
%QoS metrics for the IoT device layer include the optimum number of active sensors, sensor quality, energy consumption, data volume, trustworthiness, coverage, and mobility. Within the Cloud layer, throughput and response time are QoS requirements of the data analysis programming models, while CPU utilization, memory utilization, network latency and network bandwidth are examples of QoS of the infrastructure layer \cite{costa2017specifying}.
%Compared with the cloud-based applications, the ML-based IoT applications have similar QoS metrics such as throughput, latency, resource utilization, etc. \cite{costa2017specifying}.
%Cost is another important factor to consider in the ML-based IoT applications, which includes the cloud usage-based bill, the purchase of the IoT and edge devices as well as their maintenance fees.
%Importantly, the functionalities of the IoT applications are very diverse, making the constraints of each application very different as well.
%For example, the \emph{smart traffic routing} application is non-tolerant to latency, while accuracy is very important for a \emph{self-driving vehicle} application \cite{xu2017end}. As a result, the unsolved constraint satisfaction problems \cite{wen2019ga, wen2016dynamically, wen2016cost} in cloud computing (i.e. optimizing the deployment configuration to meet users' non-functional requirements) are harder in IoT settings. 

%At the IoT Application layer, the key requirements vary according to the type/sector for which the IoT application is developed. For example, key requirements for health-monitoring applications are robustness, durability, accuracy, precision, reliability, security, privacy, availability and responsiveness. Low latency is a key requirement in critical and real-time applications, while network utilization and energy efficiency have a high priority in less critical applications such as building automation. 
%
%Besides, budget constraint is also one of the NFR in machine learning based IoT applications. In IoT, a budget constraint represents all the combinations of devices and services that users may pay given current prices within their income. Machine learning application often requires achieving high prediction accuracy under certain budget constraint. Given a budget in terms of CPU time, the goal is to have a ranking algorithm that produces accurate ranking results within the budget. Moreover, machine learning application often requires achieving high prediction accuracy under certain budget constraint. The study of the trade-off between prediction accuracy and prediction cost becomes more popular in nowadays~\cite{snoek2012practical}.

\subsection{Resource Specification}\label{sec:resource_spe}
\label{sec:Resource Specification}
The resources in IoT domain include hardware and software. In the following section, we survey the diversity of hardware and software resources employed in IoT environment.% based on their types. 

\subsubsection{Hardware Specification}
\label{sec:Hardware Specification}
In an IoT application, hardware consists of three basic type of devices: \emph{data generating} devices, \emph{data processing} devices and \emph{data transferring} devices. 
\emph{Data generating} devices are also called ``Things'' (e.g. sensors, CCTV) and are used to collect environmental data. \emph{Data transferring} devices such as router, IoT gateway, base station are used to transfer the generated data to the \emph{data processing} devices. \emph{Data processing} devices are used to run the analytic jobs. They can be GPU, CPU and TPU servers running in cloud or ARM based edge device such as Raspberry Pi and Arduino. 
The ML-based IoT application is usually running across a fully distributed environment, such that it does not only require correct specification of the component devices alone, but also the precise interoperation between the these devices. 
\cite{singh2017create} lists fundamental aspects that may simplify hardware specification, i.e.,  processor, clock rate, general purpose input/output (GPIO), connectivity methods (Wi-Fi, Bluetooth, wired connection) and communication protocols (serial peripheral interface), universal asynchronous receiver-transmitter (UART). 

\subsubsection{Software Specification}
\label{sec:Software Specification}
In ML-based IoT applications, software specification is often categorized into three groups based on operation levels: \emph{operating system (OS)}, \emph{programming language} and \emph{platform}. % in IoT settings. 
%\zy{IoT OS provides the ability to embed the system within internet connected devices.} 
IoT OS allows users to achieve the basic behavior of a computer within internet-connected devices. The choice of OS in different layers of IoT environment depends on the hardware properties such as memory and cpu.
For example, Linux-based OS is often used in Cloud (Ubuntu) and Edge (Raspbian) with recommended minimal 4GB memory while RIOT can run in low powered IoT devices with only 10kB memory~\cite{baccelli2018riot}.
In terms of programming language, it helps. the developers to build various applications in different working environments with diverse constraints. The choice depends on the capability of devices and the purpose of the application~\cite{cabe2018iot}. 
For example in embedded IoT devices, C and C++ are the most common languages to minimize the instruction count and maximize the execution speed. 
%For Edge devices managing communication and light computation tasks, Java and Python are the most popular choices. In Cloud layer, Java and C\# are the main languages to build and develop large scale services.% with nearly unlimited computing capacity. 
%Regarding the software platform specification in IoT,
%\zy{Regarding to IoT software platform specification, it is a critical task in user specification due to the compatibility between IoT hardware and software~\cite{mineraud2016gap}.} 

The IoT software platform is a system which simplifies the development and deployment of the ML-based IoT application. 
It is an essential element of a huge IoT ecosystem which can be leveraged to connect new elements into the system.
Meanwhile, because of the heterogeneity of IoT resources, a full stack platform needs to provide the  capability to enable multi-layer technologies, such as provisioning, management and automation of IoT devices, Edge and Cloud.
IoT platform also needs to bring a set of prepared features for developers to speed up the development and management. 
For more details of the most popular OSs, programming languages and platforms in IoT domain, one can refer to \textbf{Appendix A}.
  Regarding the development platforms in ML perspectives are  discussed in section~\ref{mlframework}.

%We list several popular OSs, top 5 programming languages and some common IoT platforms using in different layers of IoT application in \zy{table~\ref{SoftwareList}}.\bin{APPENDIX} Regarding machine learning software specification, a list of popular machine learning developing tools are discussed in section~\ref{mlframework}.

%\begin{table}[t]
%\footnotesize
%\begin{tabular}{|c|l|l|l|}
%\hline
%Software Specification   & \multicolumn{1}{c|}{\textbf{Cloud}}                                                                                                  & \multicolumn{1}{c|}{\textbf{Edge}}                                                                                                                  & \multicolumn{1}{c|}{\textbf{IoT devices}}                                                                                              \\ \hline
%\multirow{6}{*}{Main OS} & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}- Ubuntu\\ - CentOS\\ - Debian\\ - RHEL\\ - Windows Server\\ - Amazon Linux\end{tabular}} & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}- Raspbian\\ - NOOBS\\ - Amazon FreeRTOS\\ - RIOT\\ - Google Fuchsia OS\\ - Windows 10 IoT\end{tabular}} & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}- Amazon FreeRTOS\\ - Contiki\\ - TinyOS\\ - RIOT\\ - Ubuntu Core\\ - Mbed OS\end{tabular}} \\
%                         &                                                                                                                                      &                                                                                                                                                     &                                                                                                                                        \\
%                         &                                                                                                                                      &                                                                                                                                                     &                                                                                                                                        \\
%                         &                                                                                                                                      &                                                                                                                                                     &                                                                                                                                        \\
%                         &                                                                                                                                      &                                                                                                                                                     &                                                                                                                                        \\
%                         &                                                                                                                                      &                                                                                                                                                     &                                                                                                                                        \\ \hline
%Programming Language     & \begin{tabular}[c]{@{}l@{}}- Java\\ - ASP.NET\\ - Python\\ - PHP\\ - Ruby\end{tabular}                                               & \begin{tabular}[c]{@{}l@{}}- Java\\ - Python\\ - C\\ - C++\\ - JavaScript\end{tabular}                                                              & \begin{tabular}[c]{@{}l@{}}- C\\ - C++\\ - Java\\ - JavaScript\\ - Python\end{tabular}                                                 \\ \hline
%Platforms                & \begin{tabular}[c]{@{}l@{}}- AWS\\ - Azure\\ - Google Cloud Platform\\ - IBM Cloud\\ - Oracle Cloud\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}- Amazon Greengrass\\ - EdgeX\\ - Cisco IOx\\ - Akraino Edge Stack\\ - Eclipse ioFog\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}- AWS IoT\\ - Azure IoT\\ - GCP IoT\\ - IBM Watson\\ - Cisco IoT cloud connect\end{tabular}                 \\ \hline
%\end{tabular}
%\caption{List of OS, programming language and platform in IoT layers}
%\label{SoftwareList}
%\end{table}


%The software includes the operating systems, programming languages and platforms.  The most commonly used operating systems for such embedded systems are Linux and UNIX-like OSs like Ubuntu Core or Android. Second, IoT software encompasses a wide range of software and programming languages from general-purpose languages like C++ and Java to embedded-specific choices like Google’s Go language or Parasail. Regarding machine learning software tools, PyTorch, TensorFlow, Scikit Learn, Keras and etc. are most popular tools. These tools are mainly developed by C++, C, Python and Java. The details of machine learning developing frameworks will be discussed in the following figure\ref{DLLibrary}. 

%\subsection{Constraints Specification}

%\zy{remove this subsection and merge the budget constraints with the non-functional requirements }

%In IoT machine learning area, constraints specification is the process of finding a solution to a set of constraints that impose conditions that the variables must specify. The solution is therefore a set of values for the variables that satisfies all the constraints. We categorise the constraints to budget constraints, energy constraints and security constraints.  

%\subsubsection{Budget Constraints}

%\subsubsection{Energy Constraints}
%The IoT device is constrained by the entity which is in physically monitoring state and the position of the entity is frequently changing without access to power. Most of the devices in the IoT are having considerable small size and are not fixed. Due to their size and frequently changing location property devices are not able to access the power all the time. So the low power consumption techniques or low power consumption schemes are made with long lasting lift for devices. 

%\subsubsection{Security Constraints}
%Security and privacy is one of the most important hurdle of the IoT and it has recently researched exhaustively. Securing IoT machine learning systems present a number of unique challenges because more and more IoT devices are developed and manufactured into the uncontrolled, complex real world. These challenges consists of IoT devices authorisation and authentication; communication security; web, mobile, and cloud applications security; high availability issue; vulnerabilities and incidents detection; vulnerabilities management and etc. 

\subsection{Challenges of user specification}\label{spec_discussion}
User specification is the first step in developing an ML-based IoT application. It captures and elicits the requirements from users and various stakeholders.
The heterogeneity of the IoT resources and environments requires comprehensive user specification to support the full stack system development.
However, existing specification languages can hardly cover multi-layer specification in both requirements and resources aspect.
In~\cite{costa2017specifying}, the authors proposed IoT-RML which allows user to specify multi-layer representation of requirements (functional and non-functional). The conflict among various stakeholders is greatly reduced while the resource level specification is not considered.
In~\cite{alqahtani2018end}, an end-to-end service level agreement specification language with a comprehensive vocabulary is proposed to provide a fine-grained level of specification of user requirements.
However, this work focuses on hardware perspective while software specification is lacking.
Regarding ML, there is no specification language that considers the complexity of the ML model.
For example, the ML tasks need to be represented precisely, thereby verifying the potential conflicts with resource specification. The developers can then choose the suitable ML algorithms to develop the models.



==> updating.tex <==
\section{Model updating}
\label{sec:updating}
xxxxx
